Magnushammer: A Transformer-Based Approach to Premise Selection

This paper presents a novel approach to premise selection, a crucial reasoning task in automated theorem proving. Traditionally, symbolic methods that rely on extensive domain knowledge and engineering effort are applied to this task. In contrast, this work demonstrates that contrastive training with the transformer architecture can achieve higher-quality retrieval of relevant premises, without the engineering overhead. Our method, Magnushammer, outperforms the most advanced and widely used automation tool in interactive theorem proving called Sledgehammer. On the PISA and miniF2F benchmarks Magnushammer achieves $59.5\%$ (against $38.3\%$) and $34.0\%$ (against $20.9\%$) success rates, respectively. By combining \method with a language-model-based automated theorem prover, we further improve the state-of-the-art proof success rate from $57.0\%$ to $71.0\%$ on the PISA benchmark using $4$x fewer parameters. Moreover, we develop and open source a novel dataset for premise selection, containing textual representations of (proof state, relevant premise) pairs. To the best of our knowledge, this is the largest available premise selection dataset, and the first one for the Isabelle proof assistant.

==> sections/introduction.tex <==
\section{Introduction}
\label{sec:intro}

\piotrm{30.12 The current intro:
\begin{itemize}
    \item (par 1) about mathematics
    \item (par 2) intro of premise selection
    \item (par 3) intro of LLM
    \item (par 4) intro of our method
\end{itemize}
Proposed structure:
\begin{itemize}
    \item (par 1) intro of premise selection and ATPs/ITPs
    \item (par 2) intro of data-driven approach and LLM --> our method
    \item (par 3) intro of our method
    \item (par 4) outro
\end{itemize}
}

Mathematics is at the core of all science. In computer science, among others, it is behind algorithms, compilers, computer chips, communication systems, computer graphics, and cryptography. Therefore, formal mathematical proofs can be used to verify the correctness of these systems \cite{leroy2009formal, klein2009sel4, kern1999formal}. Moreover, theoretical and practical aspects of omnipresent machine learning are based on calculus, linear algebra, information theory, probability theory, and other mathematical domains.  Unsurprisingly, the goal of automating reasoning about mathematical proofs is one of the fundamental problems of artificial intelligence and computer science \cite{handbook_atp, alemi2016deepmath, wang2017premise}. 

Mathematical statements are often too complex or take too much time and computational budget to prove without relying on already known theorems. Therefore, one of the fundamental aspects of automated theorem proving is \textit{premise selection}, a highly-challenging task of selecting relevant facts that can accelerate the proof and restrict the enormous search space. Premise selection can be viewed as a classification or ranking problem, and thus machine learning methods can be successfully applied \cite{alama2011premise, kaliszyk2017holstep, alemi2016deepmath, li2021graph, wang2017premise}.

Since 2017 transformers \cite{vaswani2017attention} have revolutionized Deep Learning and become omnipresent. Their application has accelerated domains such as reinforcement learning (RL) \cite{laskin2022context, chen2021decision, chen2022transdreamer, lee2022multi}, computer vision (CV) \cite{dosovitskiy2020image, caron2021emerging}, Generative Adversarial Networks (GANs) \cite{xu2021stransgan, jiang2021transgan}, Speech \cite{karita2019improving, dong2018speech}, Biology \cite{AlphaFold2021}, or even Medicine \cite{shamshad2022transformers}. Among other things, transformers stay behind the powerful language models like T5, GPT-3 or Codex \cite{raffel2019exploring, radford2021learning, chen2021evaluating}, and were the key to unlocking the long-standing problem of protein folding in DeepMind's AlphaFold work \cite{AlphaFold2021}. Finally, language models have been also successfully applied in the domain of automated theorem proving \cite{polu2020generative, jiang2022thor, jiang2021lisa, polu2022formal}. Despite the abundance of prior work and recent progress, the problems of automating mathematical reasoning and premise selection are still far from being solved.

In this paper, we introduce a neural, transformer-based, model for premise selection.  The presented solution leverages the concept of contrastive representation learning which ensures that matching statements are close in the latent space and non-matching ones are far from each other. In our approach, the Premise Selection Model is trained to embed any premise or proof state into a latent space vector. Such a method is fast and efficient for searching through large databases. However, encoding into latent space might not allow the model to catch all the details of the input statement. Simultaneously, because each premise and each proof state are encoded independently, this does not allow the model to reason about premises \textit{in the context of} the current proof state. Alternatively, one can combine a prospective premise with the current proof state and give a full textual representation to the model. Such an approach allows the model to access the full textual representation and score each premise \textit{in-context of the given proof state}. However, this approach is inefficient when the database of available facts is large. We propose to combine text similarity and representation similarity and get the best out of both worlds. Towards this, we design and implement a method named \method. The procedure is hierarchical. First, the representation similarity model selects top premises from a large database. Then the textual representations of each of the chosen premises, along with the proof state, are given to the model, and the initial ordering of the proposed facts is refined.



\paragraph{Contributions}
\begin{enumerate}
    \item We design, implement and benchmark a simple, generic, efficient, and domain-expertise-free neural model for premise selection from large databases. The proposed method outperforms state-of-the-art software, developed over years, for premise selection. Our solution achieves \maciejm{TODO final score} proof rate, whereas Sledgehammer achieves $35.0\%$.
    \item We raise the state-of-the-art success rate of the language-model-based reasoning system on PISA from $57.0\%$ to TODO :) ...
    \item We propose a method for data-mining for automated theorem proving with a focus on premise selection. We open-source the extracted data which is the largest \maciejm{Is it? Or maybe the only?} database for premise selection for ATP available. 
\end{enumerate}
\piotrm{30.12 Proposed contributions:
\begin{itemize}
    \item \method; simple, generic, efficient model for premise selection from large databases 
    \item dataset and extraction method
\end{itemize}}

==> sections/todolist.tex <==
% \section*{TODO List}


% 

{\small

% \maciejm{The example\_paper\_icml\_2023.pdf in overleaf contains detailed instructions for how to write an ICML paper. }

% \maciejm{10.01 Taken from RETRO: ``2.6. Quantifying dataset leakage exploitation
% Retro models may arguably benefit more easily from evaluation dataset leakage, i.e. the fact that we evaluate on data that were also present in the training set''. TODO: Look into retro paper and provide a similar explanation of how we filter proofs from test-theorem @SA.
% Otherwise someone can complain. We need to explain how we clean dataset and remove "test theorems".}

% \szt{08.01 Idea for a separate "Background" section which is mainly about Sledgehammer
% \begin{itemize}
%     \item Explain what is Sledgehammer on a high level - but not that high level. Mention proof reconstruction which is a complicated piece of software very few people understand. Mention that its final output is just Isabelle steps with premises, and our main goal is to skip proof reconstruction and generate those steps directly by doing tactics + premise selection. \szymona{Problem translation to requisite logics is another matter that is still an open problem, the present solutions still need improvement. The external solvers, too, are difficult to develop and need expertise from members of a narrow, specialised field.}
%     \item Say why it is important for the Isabelle community, ppl generate proofs using it, and why e.g. Lean doesn't have it?
%     \item We can also move some background stuff from introduction that we consider less important? (but honestly it would be better to remove it)
% \end{itemize}
% }

% \maciejm{This section contains a list of questions or delicate points that we should consider and address correctly in our work.}

% \piotrm{18.01 Various comments on the eval protocol commented below}
% =========== Comments on the eval protocol ===========
% \paragraph{Why is eval so slow? Iteratively trying each step...} It's not our bottleneck. PISA does not allow you to try many steps at once. In principle, we could run all of it in parallel, assuming many cores, and our method would take only 10sec.

% \paragraph{Does SH scale with timeout?} No it does not.\szymona{claiming this is suicide. Consult page 4 of Sledgehammer: Judgement Day paper. They show how SH performance changes with larger timeouts. Claiming this only shows flaws in our setup, \textbf{which we do not want} } I have the results for it. TODO: include it somewhere in the ablation or appendix.


% \begin{enumerate}
%     % \item \szt{06.01: Describe sledgehammer in a separate subsection in much detail. Emphasize how complicated it is. It is not important for the reader to understand hammer, but the background is extremely important to sell our idea. Replacing sledgehammer is the 90\% of the paper. Mention this in the new intro, but a completely separate subsection would be nice.}
%     \item Proof Rate Root Benchmark is our own benchmark. We have to ensure that it's convincing for a reader. \szt{One point would be that symbolic ATP tools like sledgehammer don't allow for intermediate proof steps so applying them for root is the only way, another supporting data point would be evaluating our method on a Thor-like setup.}
%     \item Our numerous tactics and iteration over K makes inference slow. We have to correctly describe it and emphasize that we assume a parallel computation paradigm in which total time would be the same as a single call. Nowadays it corresponds to e.g. running multiple instances of the environment in parallel. \szymona{the reality is much much better! Isabelle was designed with parallel calls in mind and handles them effortlessly [this is still being verified, waiting for mailing list guys response]}
%     \item Considering the above, how many tactics \& $K$ values we want to include? The more we do the bigger the proof rate.
%     \item \szt{We have to ensure that we convince people from different envs (lean, coq) that our method can be applied in their settings, even though there is no strong hammer and thus no partially hammer-generated data to train on. There are at least 2 points that would support this: 1) proof rate on raw AFP (not ideal as AFP also contains hammer-generated stuff) 2) dataset ablation wrt. number of train examples 3) dataset ablation wrt. tactics used? (but hammer can use anything so that's unclear)  }
% \end{enumerate}
% =========== Comments on the eval protocol ===========

}



